Managing Data Lineage of O&G Machine Learning Models: The Sweet Spot for Shale Use Case

Machine Learning (ML) has increased its role, becoming essential in several industries. However, questions around training data lineage, such as "where has the dataset used to train this model come from?"; the introduction of several new data protection legislation; and, the need for data governance requirements, have hindered the adoption of ML models in the real world. In this paper, we discuss how data lineage can be leveraged to benefit the ML lifecycle to build ML models to discover sweet-spots for shale oil and gas production, a major application in the Oil and Gas O&G Industry.

==> sections/background.tex <==
% \subsection{ProvLake}

ProvLake (Figure is a system for runtime analysis of multiworkflow data. 
ProvLake has a microservices architecture composed of three services (ProvCapturer, ProvManager, and PolyProvQueryEngine), a lightweight ProvLake library, a messaging system, and the PLView (Figure~\ref{img:provlake:architecture}).
ProvLake logically integrates and ingests multiworkflow data into a provenance database, named ProvLake Data View (PLView), ready for data analyses at runtime. 
During a multiworkflow execution, the PLView is filled with following contents:
    domain data extracted from data stored in multiple stores; 
    explict data relationships datasets distributed across the multiple stores; 
    and the multiworkflow data relationshios. 
The PLView is materialized in a DBMS.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.5\textwidth]{images/provlake_architecture.png}
  \caption{ProvLake architecture}\label{img:provlake:architecture}
\end{figure}


To populate the PLView, ProvLake Lib (which encapsulates API calls added to workflow codes) send data to the ProvCapturer, which receives data coming from the running workflows and transforms into provenance data following ProvLake's data representation which extends W3C PROV-DM \cite{provdm}. Then, the ProvCapturer sends provenance data to ProvManager which has the connectors to insert data into the DBMS managing the PLView.

To query the PLView, clients send API query requests to PolyProvQueryEngine which connects to ProvDataManager to query the PLView and employs a polystore to query data directly in the multiple stores, jointly with their provenance data.


% Prospective and Retrospective provenance


==> sections/prov-sss.tex <==
% What is SSS?
Interest in shale plays has grown substantially due to horizontal drilling and hydraulic fracturing techniques. Special interest is in shale plays previously exhausted with vertical wells that are believed to still have high potential if developed with horizontal wells. However, with drilling costs at an all time high, choosing the right locations for new wells is a crucial issue.
Therefore, identifying so called ``sweet spots'' with high potential for oil and gas is of great importance for oil companies worldwide.
\cite{bianca2019sss} describes a machine learning method that integrates heterogeneous data (well log data, production data, \ldots) to train predictive models for the identification of Sweet spot for Shale plays, henceforth, called \textit{SSS}.
Figure~\ref{img:sss:workflow} depicts SSS' workflow\footnote{Yellow boxes are data items, rounded blue boxes are activities (i.e., data transformations), and arrows represent data dependencies -- an arrow leaving a data item indicates that the following activity used it, while an arrow arriving indicates that the activity generated it.}. 

\begin{figure}[!htb]
  \centering
  \includegraphics[width=1\textwidth]{images/sss_workflow.pdf}
  \caption{Sweet Spot for Shale Workflow}\label{img:sss:workflow}
\end{figure}

SSS was implemented as a set of microservices, each responsible for one or multiple tasks in the workflow. 
%   Capturing provenance in a microservices architecture
To facilitate adoption, instead of instrumenting each microservice separately, we instrumented the reverse proxy middleware -- generating the retrospective provenance for each received request.

% Query API
Answering provenance queries, like the ones listed in Table~\ref{tab:queries}, is to find a path between two vertices in the provenance graph. For instance, to answer Q2, one needs to find a graph traversal path connecting a particular \texttt{file\_path}, an \texttt{Upload Well} activity's input, to a \texttt{ProjectTraining.trainingId}, a \texttt{Train} activity's  output. 

We noticed two distinct provenance data insertion patterns: 
    one from the normal use of the system, where users would interact with a graphical interface, 
    and another from a batch processing of historical data -- the creation of retrospective provenance data based on pre-existing SSS' database records. 
%   CQRS
Because of this requirement, we employed a Command-Query Responsibility Segregation (CQRS)~\cite{newman2015building} like approach in the access of the provenance database. 
We isolated information retrieval (query-side) from transaction (command-side) operations by having one database service for the first and another one for the second; however, we kept both servers accessing shared database. Besides, the database was replicated. In other words, considering our technology stack, our deployment included one JanusGraph for read operations, one JanusGraph for writing operations, and three Cassandras as database replicas, Figure ~\ref{img:provlake:actual} depicts the instantiated architecture. It resulted in performance gains in order of \% since batch insert operations were very frequent and were impacting queries.



\begin{figure}[!htb]
  \centering
  \includegraphics[width=1\textwidth]{images/provlake_implemented_architecture.png}
  \caption{ProvLake's architecture for the SSS use case. A HyperKnowledge Base (HKB) instantiates the PLView. Kafka was used to track the progress of asynchronous insertions. In this particular use case the ProvLakeLib was used to instrument SSS' middleware instead of its scripts. }\label{img:provlake:actual}
\end{figure}



\input{sections/queries_table.tex}

==> sections/prov_sss_experiments.tex <==
In order to justify this architectural decision we experimented varying the number or concurrent write request ({10, 100}) with a query request, the number of Cassandra replicas ({1, 3}), and two architectural configurations one service for read and write requests or read and write split into two services.  Figure 1 and 2 shows the experimental results, thus justifying our architectural decisions.

\begin{figure}[!htb]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{images/exp_split_RW_HKBase.pdf}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{images/exp_cassandras.pdf}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
\caption{(a) Box plot showing the variation of  query response time  (read) varying the number of concurrent write request (\{10, 100\}) for two configurations: (red) one service for read/write, and (blue) one service for read another service for write, dedicated services increased the throughput. (b) Box plot showing how query rezsponse is affect varying the number of Cassandra replicas (\{1, 3\}), increasing the number of Cassandra replicas increased the reading performance.}
\label{fig:fig}
\end{figure}
